Blockchain-Enabled IoV: Secure Communication and Trustworthy Decision-Making

The Internet of Vehicles (IoV), which enables interactions between vehicles, infrastructure, and the environment, faces challenges in maintaining communication security and reliable automated decisions. This paper introduces a decentralized framework comprising a primary layer for managing inter-vehicle communication and a sub-layer for securing intra-vehicle interactions. By implementing blockchain-based protocols like Blockchain-integrated Secure Authentication (BiSA) and Decentralized Blockchain Name Resolution (DBNR), the framework ensures secure, decentralized identity management and reliable data exchanges, thereby supporting safe and efficient autonomous vehicle operations.

==> scrapped.tex <==
By decentralizing identity management across multiple nodes (such as RSUs and edge servers), the system stands resilient against attacks like Sybil and Spoofing. The use of blockchain ensures that all communication routes are tamper-proof, preventing unauthorized access and ensuring the integrity of data exchanged between vehicles and infrastructure.
